Making Language Models Robust Against Negation

Negation has been a long-standing challenge for language models. Previous studies have shown that they struggle with negation in many natural language understanding tasks. In this work, we propose a self-supervised method to make language models more robust against negation. We introduce a novel task, Next Sentence Polarity Prediction (NSPP), and a variation of the Next Sentence Prediction (NSP) task. We show that BERT and RoBERTa further pre-trained on our tasks outperform the off-the-shelf versions on nine negation-related benchmarks. Most notably, our pre-training tasks yield between 1.8% and 9.1% improvement on CondaQA, a large question-answering corpus requiring reasoning over negation.

==> apptex/lama-results.tex <==
\section{Results on LAMA}
\label{app:lamaresults}

% LAMA - RoBERTa
\begin{table*}
    \centering
    \input{tables/lama.tex}
    \caption{
      We report the mean precision at $k = 1$ on the original LAMA dataset.
      The higher the precision, the better the model.
      Other than {RoBERTa} models jointly pre-trained on both tasks, 
      all our models are within $\pm$1.65\% of the vanilla models. 
      \label{tab:lama-roberta}
    }
  \end{table*}

Table~\ref{tab:lama-roberta} presents the mean precision at $k = 1$ on the original LAMA dataset. 
Except for {RoBERTa} models jointly pre-trained on both NSP and NSPP, 
all other models remain within $\pm$1.65\% of the vanilla models. 
Notably, models pre-trained on NSP and NSPP consistently outperform the vanilla models on {SQuAD} by 0.33\%-1.32\%,
with the sole exception of {BERT-base} pre-trained on NSPP, which performs 0.32\% worse.

On {GoogleRE}, the gains are less pronounced, with improvements ranging from 0.01\% to 0.65\%, 
except for {RoBERTa-base} pre-trained on NSPP, which performs 0.33\% worse. 
For ConceptNet and TREx, the models perform within $-1.65\%$ to $+0.21\%$ of the vanilla models.

It is important to note that LAMA does not contain negated instances, 
so improvements are not necessarily expected. 
However, the fact that the models remain within $\pm$1.65\% of the vanilla models, 
coupled with the substantial improvements on LAMA-neg (Table~\ref{tab:lama-neg}) 
and other corpora, 
demonstrates that the models achieve more robustness to negation while maintaining competitive performance on inputs without negation.

==> apptex/nlu-results.tex <==
\section{Results on the NLU Tasks}
\label{app:nluresults}

\begin{table*}
    \centering
    \input{tables/nluresults.tex}
    \caption{
        Results on the validation sets of natural language understanding tasks.
        All numbers are macro-averaged F1 scores.
        \label{tab:nluresults}
        }
\end{table*}

Table~\ref{tab:nluresults} presents the results on the validation sets of natural language understanding tasks. 
Following prior work, we report macro-averaged F1 scores on the validation sets as some test labels are not publicly available. 
The results demonstrate that further pre-training consistently improves performance on instances containing negation or, at worst, causes a negligible decline 
(a marginal 0.01\% decrease with {RoBERTa-base} on WSC.)
On average, pre-training yields a 3.11\% improvement across all tasks.
Notably, the most significant improvements are observed on WiC with base models
(achieving an average increase of 7.5\%) and on WSC with large models (where performance improves by 6.0\% on average.) 
Importantly, all models pre-trained on NSP or NSPP outperform off-the-shelf versions on important instances in QNLI, 
with the only exceptions being {BERT-large} pre-trained on either NSPP or NSP. 

